LogiAgent: Automated Logical Testing for REST Systems with LLM-Based Multi-Agents

Automated testing for REST APIs has become essential for ensuring the correctness and reliability of modern web services. While existing approaches primarily focus on detecting server crashes and error codes, they often overlook logical issues that arise due to evolving business logic and domain-specific requirements. To address this limitation, we propose LogiAgent, a novel approach for logical testing of REST systems. Built upon a large language model (LLM)-driven multi-agent framework, LogiAgent integrates a Test Scenario Generator, API Request Executor, and API Response Validator to collaboratively generate, execute, and validate API test scenarios. Unlike traditional testing methods that focus on status codes like 5xx, LogiAgent incorporates logical oracles that assess responses based on business logic, ensuring more comprehensive testing. The system is further enhanced by an Execution Memory component that stores historical API execution data for contextual consistency. We conduct extensive experiments across 12 real-world REST systems, demonstrating that LogiAgent effectively identifies 234 logical issues with an accuracy of 66.19%. Additionally, it basically excels in detecting server crashes and achieves superior test coverage compared to four state-of-the-art REST API testing tools. An ablation study confirms the significant contribution of LogiAgent's memory components to improving test coverage.

==> sections/approaches/ARG.tex <==
%本节内容被移动至test scenario agent中%

%1.json/yaml 不是给LLM设计的，不利于其更好的理解文档%
%2.上下文可能很长%
%3.没有包含API之间可能的关联关系%
Although large language models (LLMs) are capable of understanding raw OpenAPI~\cite{openapi_spec} documentation, the typical formats of OpenAPI documentation (JSON or YAML) propose a challenge for LLMs to fully understanding it, as these formats are not naturally compatible with LLMs' language processing mechanisms, they may limit the model’s ability to interpret and use the information effectively~\cite{PromptFormatting}.
Additionally, OpenAPI documentation often contains long contextual information, which makes it difficult for LLMs to accurately understand the details of the specification.
Furthermore, the lack of explicit representation of relationships between APIs makes it challenging for LLMs to process complex API interactions and dependencies effectively.

%介绍API Relationship Graph的构成与构建方式%
To address previous challenges, we propose the API Relationship Graph(ARG), a structured representation of the API system, aims to enhance the understanding of the LLMs for the under-test REST API systems. 


\subsubsection{Graph Construction} The ARG is constructed as follows:
\textbf{Nodes:} Represents an API, have following attributes:
\begin{itemize}
    \item \textbf{API Method:} HTTP methods of the API (e.g., GET, POST, PUT and DELETE) .
    \item \textbf{API Path:} HTTP URL path of the API (e.g., \textit{/api/pet}) .
    \item \textbf{Raw API Content:} Origin content of the API in the OpenAPI documentation, typically including request parameters, request body, response codes, response body, etc. According to~\cite{PromptFormatting}, to achieve optimal performance, we convert the raw API content into a structured Markdown format before feeding it to GPT-4 series models.
\end{itemize}


\textbf{Edges:} Represent potential relationships between APIs. Our core approach is to leverage LLMs to assess whether two APIs are related by analyzing their descriptions. 
However, as the number of APIs increases, the number of pairwise comparisons required for constructing the graph grows exponentially, making direct comparisons impractical.
To address this, we adopt a two-step strategy:

\begin{itemize}
\item \textbf{Preliminary Filtering:} We first compute the cosine similarity between the embeddings of two APIs. The embeddings are generated using OpenAI's text-embedding model~\cite{openai_embedding}, which converts API metadata into numerical vector representations.
\item \textbf{Further Validation:} For API pairs that pass the initial filtering, we apply GPT to determine whether a meaningful relationship exists between them, ensuring a refined and efficient selection process.
\end{itemize}


\subsubsection{Random Walk Strategies}

In systems with a large number of APIs, providing all apis to the LLM can overwhelm the context, thereby compromising the quality of the generated test scenarios. 

To address this issue, whenever a test scenario needs to be generated, we apply a random walk strategy to the API Relationship Graph (ARG) to select a subset of APIs based on their relational edges in the graph.
This approach ensures the generation of more effective and relevant test scenarios.
